Attribute Alignment: Controlling Text Generation from Pre-trained Language Models

Large language models benefit from training with a large amount of unlabeled text, which gives them increasingly fluent and diverse generation capabilities. However, using these models for text generation that takes into account target attributes, such as sentiment polarity or specific topics, remains a challenge. We propose a simple and flexible method for controlling text generation by aligning disentangled attribute representations. In contrast to recent efforts on training a discriminator to perturb the token level distribution for an attribute, we use the same data to learn an alignment function to guide the pre-trained, non-controlled language model to generate texts with the target attribute without changing the original language model parameters. We evaluate our method on sentiment- and topic-controlled generation, and show large performance gains over previous methods while retaining fluency and diversity.

==> tables/oppo_sent.tex <==
\begin{table*}[t]
\small
  \centering
  \begin{tabular} {  p{1.2cm} | p{14cm}  } 
    \hline
 \textbf{Target} & \textbf{Generated Text}\\
 \hline
 positive &\underline{The food is awful} but the service is amazing! The takeout is amazing! However, for me, a small, cozy restaurant that is a small institution in a small town I'm so glad that they are planning on ...\\
 \hline
 negative &\underline{The food is amazing}!! We didn't want to bring it home as the night before, but we can't afford the honey pot cost so we ended up throwing in our own trail mix as well as having ...\\
 \hline
  \end{tabular}
  \caption{Adversarial sentiment control examples generated from the proposed alignment function with Bayes disentanglement (ACB) where the prompt has a strong opposite sentiment. Similar to Table~\ref{table:control_example}, the results here are selected by a sentiment classifier (not cherry-picked).}
  
\label{table:oppo_sent}
\end{table*}
